Augmenting Interpretable Models with LLMs during Training

Recent large language models (LLMs) have demonstrated remarkable prediction performance for a growing array of tasks. However, their proliferation into high-stakes domains (e.g. medicine) and compute-limited settings has created a burgeoning need for interpretability and efficiency. We address this need by proposing Augmented Interpretable Models (Aug-imodels), a framework for leveraging the knowledge learned by LLMs to build extremely efficient and interpretable models. Aug-imodels use LLMs during fitting but not during inference, allowing complete transparency and often a speed/memory improvement of greater than 1,000x for inference compared to LLMs. We explore two instantiations of Aug-imodels in natural-language processing: (i) Aug-GAM, which augments a generalized additive model with decoupled embeddings from an LLM and (ii) Aug-Tree, which augments a decision tree with LLM feature expansions. Across a variety of text-classification datasets, both outperform their non-augmented counterparts. Aug-GAM can even outperform much larger models (e.g. a 6-billion parameter GPT-J model), despite having 10,000x fewer parameters and being fully transparent. We further explore Aug-imodels in a natural-language fMRI study, where they generate interesting interpretations from scientific data. All code for using Aug-imodels and reproducing results is made available on Github.

==> tabs/expansion_examples_full.tex <==
\begin{tabular}{p{0.01\textwidth} p{0.1\linewidth} p{0.74\linewidth} p{0.05\textwidth} p{0.05\linewidth} p{0.05\linewidth}}
\toprule
                                                                          &   Keyword &                                                                                    Example expansion &  \# Expansions &  Mean expansions &  \# Expansion candidates \\
\midrule
 \parbox[c]{1mm}{\multirow{6}{*}{\rotatebox[origin=c]{90} {Rotten tomatoes}}} &      dull & dreary, uninteresting, lackluster, listless, lifeless, uninspired, wearisome, drab, joylessly, un... &            46 &             12.4 &                      92 \\
                                                                                  &       bad & unpleasant, dire, despicable, terrible, heinous, disgusting, vile, putrid, atrocious, nasty, poor... &            40 &             16.4 &                      99 \\
                                                                                  &      just & solely, simply, unexplained, primarily, merely, inevitably, only, undeniably, strictly, explicit,... &            32 &              5.8 &                      86 \\
                                                                                  &      like & favour, attachment, sentiment, interest, cherish, sympathy, sympathizing, taste, passion, admirin... &            31 &              4.8 &                      95 \\
                                                                                  &     silly & off the wall, farcical, humor, ridiculous, lunacy, unbalanced, nonsensical, slapstick, silliness,... &            15 &              8.3 &                      99 \\
                                                                                  &      only &               alone, solely, strictly, paramount, impenetrable, particular, undisputed, merely, just &            15 &              5.1 &                      65 \\
             \midrule 
 \parbox[c]{1mm}{\multirow{6}{*}{\rotatebox[origin=c]{90} {Emotion}}} & miserable & gloomy, disillusioned, pathetic, doomed, agonized, despairing, pointless, despondent, discouraged... &            31 &             27.2 &                      96 \\
                                                                                  &     sorry & embarrassed, sorrowful, remorseful, excuse, unsatisfied, guilt, regretful, forgive, apologies, un... &            27 &              9.7 &                      96 \\
                                                                                  &      more &           heightened, improved, extra, prolonged, added, additional, uplifted, accumulated, advanced &            25 &              5.4 &                      52 \\
                                                                                  & exhausted &                                                       spent, weary, worn out, tired, all in, drained &            17 &              3.2 &                      87 \\
                                                                                  &      very &                                                                                    extremely, highly &            11 &              1.5 &                      88 \\
                                                                                  &  stressed &                                       strain, anxious, frazzled, worn out, exhausted, drained, weary &             9 &              3.5 &                      99 \\
                \midrule 
 \parbox[c]{1mm}{\multirow{6}{*}{\rotatebox[origin=c]{90} {SST2}}} &      good & fine, highly, solid, worthy, pleasing, satisfactory, outstanding, honorable, unwavering, valuable... &            54 &             10.5 &                      91 \\
                                                                                  &      best & most remarkable, outstanding, superb, flawless, splendid, superlative, exceptional, impeccable, f... &            40 &             14.5 &                      90 \\
                                                                                  &     funny & amiable, whimsicality, comical, comic, quirky, zany, playful, hilarious, quirkiness, jovial, witt... &            39 &             15.2 &                      96 \\
                                                                                  &      love & delight, devoted, respect, tenderness, enthusiasm, loyalty, enthusiastically, lovingly, compassio... &            34 &             20.0 &                      89 \\
                                                                                  &  the best &        splendid, exquisite, unparalleled, magnificent, outstanding, finest, superlative, exceptional &            32 &              3.2 &                      87 \\
                                                                                  &     heart & respect, true love, tenderly, love affair, affectionate, loyalty, heartstrings, ardor, devotion, ... &            30 &              6.9 &                      84 \\
\midrule 
 \parbox[c]{1mm}{\multirow{6}{*}{\rotatebox[origin=c]{90} {Financial phrasebank}}} & increased &                                                                                widened, consolidated &            11 &              0.9 &                      92 \\
                                                                                  &      fell &                                slipped, slumped, diminished, plunged, dropped, weakened, lost ground &             6 &              1.8 &                      84 \\
                                                                                  &      grew &                                                                                    increased, surged &             5 &              1.0 &                      97 \\
                                                                                  &   finnish &                                                                                             helsinki &             2 &              1.0 &                      79 \\
                                                                                  &   percent &                                                                                                share &             2 &              0.7 &                      78 \\
                                                                                  &    supply &                                                                                   supplier, delivery &             2 &              1.5 &                      98 \\
\bottomrule
\end{tabular}


==> tabs/fmri_main.tex <==
\begin{tabular}{lccc}
\toprule
          &  \makecell{$\rho$\\(all)}&  \makecell{$\rho$\\(top 1\%)} &  \makecell{$\rho$\\(top 5\%)} \\ %&  \makecell{Percentage voxels\\($\rho > 0$)} &  \makecell{Percentage voxels\\($\rho > 0.2$)} \\
\midrule
\textbf{\method} &   \textbf{0.062} &                         \textbf{0.586} &                         \textbf{0.489} \\ %&                                       \textbf{58\%} &                                         \textbf{20.8\%} \\
          BERT &   0.053 &                         0.524 &                         0.429         \\ %                 &             56.2\% &                                         11.7\% \\
       % Eng1000 &   0.041 &                         0.529 &                         0.439 \\ %&                                       53.3\% &                                         17.0\% \\
         % GloVe &   0.044 &                         0.521 &                         0.426 \\ %&                                       57.1\% &                                         15.3\% \\
\bottomrule
\end{tabular}

==> tabs/variation_results.tex <==
\begin{tabular}{ccccc}
\toprule
 & Financial phrasebank &      Rotten tomatoes &                 SST2  &              Emotion \\ %&         Tweet (Hate) \\
\midrule
\makecell{BERT finetuned}                  &  \textbf{92.8\%} $\pm$ 0.37\% &  \textbf{81.6\%} $\pm$ 0.05\% &   86.9\% $\pm$ 0.1\% &  \textbf{89.5\%} $\pm$ 0.03\% \\ % &   72.6\% $\pm$ 0.2\% \\
BERT                                       &  84.1\% $\pm$ 0.08\% &  78.1\% $\pm$ 0.16\% &  82.8\% $\pm$ 0.27\% &  67.1\% $\pm$ 0.06\% \\ %&  \textbf{73.5\%} $\pm$ 0.12\% \\
DistilBERT finetuned                      &  85.8\% $\pm$ 0.34\% &  78.5\% $\pm$ 0.34\% &  81.7\% $\pm$ 0.07\%  &  68.8\% $\pm$ 0.11\% \\ %&   72.7\% $\pm$ 0.2\% \\
DistilBERT                                 &  81.7\% $\pm$ 0.34\% &  79.8\% $\pm$ 0.08\% &   86.8\% $\pm$ 0.1\%  &  87.5\% $\pm$ 0.11\% \\ %&  \textbf{73.5\%} $\pm$ 0.19\% \\
RoBERTa finetuned                                 & 77.8\% $\pm$ 0.31\%	 &  \textbf{83.6\% }$\pm$ 0.03\%	 &   \textbf{89.1\%} $\pm$ 0.24\%	  &  88.5\% $\pm$ 0.19\%		 \\ %&  \textbf{73.5\%} $\pm$ 0.19\% \\
\bottomrule
\end{tabular}
